Evolution of the UV slope of galaxies at cosmic morning (z > 4): the properties of extremely blue galaxies

We present an analysis of the UV continuum slope, beta, using a sample of 733 galaxies selected from a mixture of JWST ERS/GTO/GO observational programs and with z > 4. We consider spectroscopic data obtained with the low resolution PRISM/CLEAR NIRSpec configuration. Studying the correlation of beta with M_UV we find a decreasing trend of beta = (-0.056 +- 0.017) M_UV - (3.01 +- 0.34), consistent with brighter galaxies having redder beta as found in previous works. However, analysing the trend in separate redshift bins, we find that at high redshift the relation becomes much flatter, consistent with a flat slope. Furthermore, we find that beta decreases with redshift with an evolution as beta = (-0.075 +- 0.010) z - (1.496 +- 0.056), consistent with most previous results that show a steepening of the spectra going at higher z. We then select a sample of galaxies with extremely blue slopes (beta < -2.6): such slopes are steeper than what is predicted by stellar evolution models, even for dust free, young, metal poor populations, when the contribution of nebular emission is included. We select 51 extremely blue galaxies (XBGs) and we investigate the possible physical origin of their steep slopes, comparing them to a sub-sample of redder galaxies (matched in redshift and M_UV). We find that XBGs have younger stellar populations, stronger ionization fields, lower dust attenuation, and lower but not pristine metallicity (~ 10% solar) compared to red galaxies. However, these properties alone cannot explain the extreme beta values. By using indirect inference of Lyman continuum escape, using the most recent models, we estimate escape fractions f_esc > 10% in at least 25% of XBGs, while all the red sources have smaller f_esc. A reduced nebular continuum contribution as due to either a high escape fraction or to a bursty star-formation history is likely the origin of the extremely blue slopes.

==> abstract.tex <==
[DRAFT] In this work we present an analysis of the ultraviolet (UV) continuum slope, $\beta$, using a sample of 733 galaxies selected from JWST ERS/GTO/GO observations listed in the CEERS and JADES databases (further integrated with galaxies taken from the DJA online repository), with $z > 4$. We considered only spectroscopic data obtained with the low resolution ($R \sim 30-300$) PRISM/CLEAR NIRSpec configuration. The estimate of $\beta$ from spectroscopic data instead of a photometric evaluation has several advantages since it allows for better characterizations of spectral features and effects that might bias $\beta$ (caused for example by bright UV rest-frame emission lines, or by Lyman-$\alpha$ Damping Wing absorption, both of which we investigate in our work). Studying the correlation of $\beta$ with $M_{UV}$ we found a general decreasing trend of $\beta = (-0.056\pm0.017)M_{UV}+(-3.01\pm0.34)$, consistent with brighter galaxies presenting redder $\beta$ values. Compared to other works, the shallower trend might be due to the contribution of a population of red objects in the faint end that were probably missed in previous observations. Furthermore, we found a negative trend between $\beta$ and $z$, $\beta = (-0.075\pm0.010)z + (-1.496 \pm 0.056)$, consistent with most previous results that show a steepening of the spectra going at higher $z$ (even if we obtain a slight positive normalization offset of $\sim 0.1$ emerging towards higher redshift, where we have a poorer statistics). The physical interpretation of ultra blue galaxies ($\beta < -2.6$) is one of the main open problems regarding the structure and evolution of high redshift galaxies. Thanks to our spectroscopic-based analysis, we selected 51 extremely blue galaxies (XBGs) and we investigated the possible physical origin of their steep slope, comparing them to another sub-sample of redder galaxies (matched in $\Delta z = \pm 0.5$ and $M_{UV} = \pm 0.2$). Overall, our findings suggest that XBGs have younger stellar populations, stronger ionization fields, lower dust attenuation, and lower metallicity ($\sim 10\% Z_\odot$) compared to red galaxies. We furthermore conclude that the only physical effect that can significantly lower $\beta$ bluer than $-2.6$ is a reduced contribution of the nebular continuum emission, hence a significant leakage of ionizing radiation. By using indirect estimates using the most recent models we estimate values for the escape fraction $f_{esc} > 10\%$ in $50\%$ of the XBGs, extending to $f_{esc} \geq 50\%$ in a subset XX of them.
